Towards Theoretical Understanding of Transformer Test-Time Computing: Investigation on In-Context Linear Regression

Using more test-time computation during language model inference, such as generating more intermediate thoughts or sampling multiple candidate answers, has proven effective in significantly improving model performance. This paper takes an initial step toward bridging the gap between practical language model inference and theoretical transformer analysis by incorporating randomness and sampling. We focus on in-context linear regression with continuous/binary coefficients, where our framework simulates language model decoding through noise injection and binary coefficient sampling. Through this framework, we provide detailed analyses of widely adopted inference techniques. Supported by empirical results, our theoretical framework and analysis demonstrate the potential for offering new insights into understanding inference behaviors in real-world language models.

==> ArXiv/tex/algorithm.tex <==
\section{Scaling Test-time Computation for In-Context Regression}\label{sec:_test_time_computing_framework}

In this section, we introduce our theoretical framework for studying sampling-based test-time computing of transformers (Section~\ref{subsec:_transformer_test_time_compute}) through the task of in-context linear regression (Section~\ref{subsec:_theoretical_task}).
We present our framework in Section~\ref{subsec:_theoretical_framework}. 
After that, we study two instances of the in-context linear regression task \eqref{eq:_in_context_linear_regression}, depending on the types of the task prior $p_{\wb}$, to design concrete sampling algorithms for sampling-based transformer inference.  
In Sections~\ref{subsec:_continuous}, we consider the case where the task coefficient $\wb^{\ast}$ is continuous and is from a Gaussian prior.
In Section~\ref{subsec:_binary}, we study the case where $\wb^{\ast}$ is binary and $k$-sparse.

\subsection{A Theoretical Framework for Study of Test-Time Computation}\label{subsec:_theoretical_framework}

We begin by noticing that most of the existing prior works on in-context linear regression by transformers are \emph{incapable} for studying sampling-based test-time computing due to the lack of (i) randomness of the output of the transformer architecture they study; (ii)  chain-of-thought (CoT) style multi-step reasoning in their outputs. 
In order to handle such challenges, we explicitly construct an inference mechanism that involves both randomness and auto-regressive CoT reasoning to solve in-context linear regression tasks.

Specifically, motivated by the recent work of \cite{anonymous2025transformers}, we consider the specific goal of \emph{in-context coefficient prediction}, where the final output of the transformer reasoning path is a prediction $\widehat{\wb}$ of the task coefficient $\wb^{\ast}$.
The transformer could output different stochastic paths of reasoning towards a more and more precise prediction of the truth $\wb^{\ast}$, and different sampling-based test-time computing techniques correspond to how to aggregate these reasoning paths.
In the following part of this section, we introduce the details of the input format, transformer architecture, and the new inference mechanism based on sampling that allows for theoretical investigation of sampling-based test-time computing.

\paragraph{Inputs and transformer architecture.}
Given the in-context dataset $(\xb_1,y_1,\cdots,\xb_n,y_n)$, the prompt to the transformer model (defined later) is in the following format, 
\begin{align}
    \Hb_0 = \left(\begin{matrix}
        \xb_1&\cdots & \xb_n &\boldsymbol{0} \\
        y_1&\cdots&y_n& 0 \\
        \boldsymbol{0}&\cdots&\boldsymbol{0}&\wb_0\\
        0&\cdots&0&1
    \end{matrix}\right) := \left(\begin{matrix}
        \Xb^\top & \boldsymbol{0}\\
        \yb^\top & 0 \\
        \boldsymbol{0} & \wb_0 \\
        \boldsymbol{0} & 1
    \end{matrix}\right) \in\RR^{d_e\times (n+1)},\label{eq:_input}
\end{align}
where the dimension of the embedding $d_e = 2d+2$. 
We denote $\Xb^\top = (\xb_1,\cdots,\xb_n)\in\RR^{d\times n}$ as the collection of covariates, and denote $\yb^\top = (y_1,\cdots,y_n)\in\RR^{1\times n}$  as the collection of labels.
Also, we input an initial guess of the coefficient, denoted by $\wb_0$, and we assume it to be $\boldsymbol{0}$ without loss of generality.
We remark that such a prompt embedding format which separates the space of data and the space of weight predictions follows the convention of \cite{bai2024transformers, anonymous2025transformers} in order to facilitate theoretical analysis.

The model we consider is a one-layer self-attention module equipped with residual connection \citep{von2023transformers, zhang2023trained, ahn2023linear, anonymous2025transformers}. 
Specifically, we define 
\begin{align}
    \mathtt{TF}_{\theta}(\Hb):=\Hb + \Vb\Hb\cdot\frac{\Hb^\top \Wb \Hb}{n}:\RR^{d_e\times \ast}\mapsto\RR^{d_e\times \ast}.\label{eq:_transformer}
\end{align}
where $\theta = \{\Vb,\Wb\}$ is the collection of the parameters. 
Here $\Vb\in\RR^{d_e\times d_e}$ represents the consolidation of the projection and value matrices in a standard transformer block, and $\Wb\in\RR^{d_e\times d_e}$ denotes the consolidation of the key and query matrices. 
Intuitively, the model $\mathtt{TF}_{\theta}$ takes as input an embedding matrix with arbitrary number of columns of dimension $d_e$ and outputs the transformed embedding for each token.

\paragraph{Sampling-based auto-regressive inference mechanism.}
With the model \eqref{eq:_transformer} and the prompt \eqref{eq:_input}, we consider the following mechanism of auto-regressive inference that mimics a real LLM (Section~\ref{subsec:_transformer_test_time_compute}).
\begin{definition}[Inference mechanism]\label{def:_inference_mechanism}
Given an input prompt embedding matrix $\Hb_0$, for each $\ell\in\NN$, we iteratively sample the embeddings for the next token as following,
\begin{itemize}
    \item Compute $\widetilde{\Hb}_{\ell} = \mathtt{TF}_{\theta}(\Hb_{\ell})$ where $\mathtt{TF}_{\theta}(\Hb_{\ell})$ is defined in \eqref{eq:_transformer};
    \item Extract $\widetilde{\hb}_{\ell}$ from the last column of $\widetilde{\Hb}_{\ell}$, i.e., $\widetilde{\hb}_{\ell} = (\widetilde{\Hb}_{\ell})_{:,-1}$;
    \item Sample the embedding for the next token via $\mathtt{Sampling\_Alg}$, i.e., $\hb_{\ell+1} \leftarrow \mathtt{Sampling\_Alg}(\widetilde{\hb}_{\ell})$; 
    \item Concatenate to obtain the embedding matrix for the new sequence of length $\ell+1$, i.e., $\Hb_{\ell+1} = (\Hb_{\ell}, \hb_{\ell+1})$.
\end{itemize}
\end{definition}
Here $\mathtt{Sampling\_Alg}(\cdot)$ is an algorithm to be determined that can prescribe the distribution of the next token (embedding) given the last token's embedding output by the transformer.
The  output after $t$ iterations of the above mechanism is a joint result of the transformer model and the sampling algorithm.

Towards the goal of in-context weight prediction for \eqref{eq:_in_context_linear_regression}, we first introduce the following proposition, which shows that the transformer architecture together with a proper sampling algorithm  $\mathtt{Sampling\_Alg}(\cdot)$ can implement variants of \emph{noisy gradient descent}.


\begin{proposition}[Transformer implements noisy GD]\label{prop:_construction}
    There exists a transformer instance of \eqref{eq:_transformer} denoted by $\mathtt{TF}_{\theta_{\mathtt{GD}}}$ and a type of sampling algorithm $\mathtt{Sampling\_Alg}$ such that given prompt $\Hb_0$ defined in  \eqref{eq:_input}, the output embedding after $t$ iterative generations $\Hb_t$ according to Definition~\ref{def:_inference_mechanism} satisfies 
    \begin{align}
        (\Hb_t)_{:,n+\ell} = \left(\begin{matrix}
            \boldsymbol{0}\\
            0\\
            \wb_{\ell}\\
            1
        \end{matrix}\right),\quad \wb_{\ell} \sim p\left(\,\cdot\,\middle|\wb_{\ell-1} - \frac{\eta}{n}\cdot \Xb^\top\big(\Xb \wb_{\ell-1}-  \yb\big)\right),\quad \forall 1\leq \ell\leq t,
    \end{align}
    where the conditional distribution $p(\cdot|\cdot )$ is specified by the sampling algorithm $\mathtt{Sampling\_Alg}$.
\end{proposition}

\begin{proof}[Proof of Proposition~\ref{prop:_construction}]
    This proposition is mainly motivated by a recent work of \cite{anonymous2025transformers}.
    Please refer to Appendix~\ref{subsec:_proof_prop_construction} for a detailed proof of Proposition~\ref{prop:_construction}
\end{proof}

Proposition~\ref{prop:_construction} shows that the above inference mechanism is able to explicitly implement gradient-based iterative algorithms to predict the regression coefficient $\wb^{\ast}$.
We define the prediction of the regression coefficient after $t$ reasoning steps of one reasoning path as $\wb_t:=(\Hb_t)_{d+2:2d+1, n+t}$.
One special case of Proposition~\ref{prop:_construction} is a transformer that explicitly performs standard multi-step gradient descent (GD) \citep{anonymous2025transformers}, i.e., $p(\cdot|x) = \delta_x(\cdot)$, so that the final prediction of the regression coefficient after $t$ reasoning steps is given by\footnote{\cite{anonymous2025transformers} considers transformer CoT reasoning for in-context-linear regression with \emph{noiseless} labels, but here we allow the existence of label noise.}
\begin{align}
    \wb_{\mathtt{GD}} :=(\Hb_t)_{d+2:2d+1, n+t} = \left(\Ib_d - \left(\Ib_d - \frac{\eta}{n}\cdot \Xb^\top\Xb\right)^t\right)\Xb^\top (\Xb\Xb^\top)^{-1}\yb.\label{eq:_w_gd}
\end{align}

To theoretically understand the effectiveness of more sophisticated sampling-based test-time computing techniques, e.g., Best-of-N and majority vote, we go beyond \eqref{eq:_w_gd} and consider sampling algorithms that does introduce certain randomness into the reasoning path (see Sections~\ref{subsec:_continuous} and \ref{subsec:_binary}).
We conclude and formalize these test-time computing methods we study in this paper as following.

% To this end, in the rest of the paper, we focus on the transformer and sampling algorithms satisfying Proposition~\ref{prop:_construction} and consider the following broader types of test-time computing techniques.


\begin{definition}[Sampling-based test-time computing techniques]\label{def:_test_time_computing}
    Given a transformer $\mathtt{TF}_{\theta}$ and a sampling algorithm that jointly satisfies Proposition~\ref{prop:_construction}, together with an prompt embedding matrix $\Hb_0$ in \eqref{eq:_input}, a CoT reasoning length limit $t\in\NN_+$, and a sampling budget $N\in\NN_+$, we consider the following computing methods:
    \begin{itemize}
        \item Generate $N$ random predictions of the regression coefficient as $\{\wb^{(j)}_t\}_{j=1}^N$, where for each $j\in[N]$ the prediction is extracted from $(\Hb_t)_{d+2:2d+1, n+t}$ and $\Hb_t$ is independently sampled by  Definition~\ref{def:_inference_mechanism}.
        \item Aggregate the $N$ random outcomes $\{\wb^{(j)}_t\}_{j=1}^N$ by using one of the following options:
        \begin{enumerate}
            \item Sample average: $\wb_{\mathtt{avg}}:=N^{-1}\cdot \sum_{j=1}^N\wb^{(j)}_t$;
            \item Best-of-N: $\wb_{\mathtt{BoN}}:=\argmax_{\{\wb^{(j)}_t\}_{j=1}^N}R(\wb^{(j)}_t)$ where $R(\cdot):\RR^d\mapsto\RR$ is certain reward function;
            \item Majority vote: 
            $\wb_{\mathtt{mv}}:=\argmax_{\{\wb^{(j)}_t\}_{j=1}^N}\mathtt{Occur}(\wb^{(j)}_t)$, where $\mathtt{Occur}(\cdot):\RR^d\mapsto\NN$ is a proper function that counts the occurrence of the input;
        \end{enumerate}
    \end{itemize}
\end{definition}


In the following two subsections, we instantiate the in-context linear regression task \eqref{eq:_in_context_linear_regression} to more concrete task priors, and investigate the effectiveness and the scaling law of the above test-time computing techniques. 
We also remark that in this paper we assume the existence of a transformer satisfying Proposition~\ref{prop:_construction} without explicitly training such one from scratch, which is left as an interesting future work.


\subsection{Case Study 1: In-context Linear Regression with Continuous Coefficient}\label{subsec:_continuous}

The first type of tasks we consider is standard in-context linear regression with continuous regression coefficient sampled from a Gaussian distribution, i.e., $p_{\wb} = \cN(\boldsymbol{0}, \omega^2\cdot \Ib_d)$.
For this case, the specific type of sampling algorithms $\mathtt{Sampling\_Alg}$ we study is concluded in Algorithm~\ref{alg:_sampling_alg_continuous}.

\begin{algorithm}[H]
\caption{Sampling algorithm for in-context linear regression with continuous coefficient}\label{alg:_sampling_alg_continuous}
\begin{algorithmic}[1]
  \STATE \textbf{Input:} token embedding $\widetilde{\hb}$, noise level $\sigma\geq 0$, noise transformation function $\phi_\cdot(\cdot):\RR^d\times\RR^d\mapsto\RR^d$.
  \STATE Extract the coefficient $\widetilde{\wb}$ from $\widetilde{\hb}$, i.e., $\widetilde{\wb} = (\widetilde{\hb})_{d+2:2d+1}$ (see Proposition~\ref{prop:_construction})
  \STATE Sample a noise vector $\boldsymbol{\xi} \sim \mathcal{N}(\boldsymbol{0}, \sigma^2 \cdot \Ib_d)$ \\
  \STATE Define $\wb \leftarrow \widetilde{\wb} + \phi_{\bxi}(\widetilde{\wb})$ \\
  \STATE \textbf{Output:} $\hb:=(\boldsymbol{0}, 0, \wb, 1)^\top$.
\end{algorithmic}
\end{algorithm}

Under sampling method Algorithm~\ref{alg:_sampling_alg_continuous}, Proposition~\ref{prop:_construction} is satisfied with $ x'\sim p(\cdot|x)$ given by $x'  = x + \phi_{\bxi}(x)$ for a Gaussian random seed $\bxi$ and some noise transformation function $\phi_{\bxi}$.
Recall that by Proposition~\ref{prop:_construction}, $\widetilde{\wb}$ output by the transformer is performing one-step gradient descent from the last prediction.
The intuition of studying Algorithm~\ref{alg:_sampling_alg_continuous} is that such a noisy version of the gradient descent could allow exploration of the loss landscape, and we aim to investigate whether  the test-time computing techniques in Definition~\ref{def:_test_time_computing} could properly aggregate the random gradient-based paths to achieve a better prediction than vanilla multi-step GD \eqref{eq:_w_gd} via less overfitting.
In this paper, we investigate the following two concrete and simple examples of the noise transformation function $\phi_{\bxi}$.
Potential future works could investigate other types of $\phi_{\bxi}$.

\begin{example}[Constant noise transformation function]\label{exp:_constant}
    $\phi_{\bxi}(\wb):=\bxi$, which does not depend on the input predicted weight $\wb$ and is homogeneous in distribution across different reasoning steps.
\end{example}


\begin{example}[Linear noise transformation function]\label{exp:_linear}
    $\phi_{\bxi}(\wb):= \bxi\bxi^\top\wb$, which is linear in the input predicted weight $\wb$ such that the sampling distribution has different shape based upon the current decoding result.
\end{example}

With Algorithm~\ref{alg:_sampling_alg_continuous}, we study the following test-time computing techniques in Definition~\ref{def:_test_time_computing}.

\paragraph{Baseline: multi-step GD with CoT \eqref{eq:_w_gd}.} 
The baseline is a transformer implementing a vanilla GD, without using Algorithm~\ref{alg:_sampling_alg_continuous} but directly using one-step GD prediction as the next token \citep{anonymous2025transformers}. 
As we can see quickly, such a deterministic method can result in overfitting to the in-context dataset since the label is noisy, and thus resulting in performance worse than sampling-based methods.

\paragraph{Sample average.} We consider sample average of the prediction from $N$ independent reasoning paths. The resulting prediction after $N$ sampling paths of  length $t$ is denoted by $\wb_{\mathtt{avg}}$ (See option 1 in Definition~\ref{def:_test_time_computing}).

\paragraph{Best-of-N.} We also consider the method of BoN when the prior of the regression coefficient is sparse. 
That is, when the true coefficient $\wb^{\ast}$ is a continuous vector in $\RR^d$ with $k$ non-zero coordinates, we apply BoN as the aggregation method, with reward function $R(\wb) := -\|\wb\|_1$.
We denote the resulting  prediction after $N$ sampling paths of  length $t$ by $\wb_{\mathtt{BoN}}$ (see option 2 in Definition~\ref{def:_test_time_computing}).



\paragraph{}

\textcolor{purple}{[Present numerical experiment results of (i) GD (ii) constant noise with averaging/BoN; (iii) linear noise with averaging/BoN.]}



\subsection{Case Study 2: In-context Binary Sparse Linear Regression}\label{subsec:_binary}

We also consider another case in which the coefficient is a sparse binary vector, denoted as $\wb^* \in \{0,1\}^d$ with $||\wb^*||_0 = k < d$. In this case, we consider the following sampling algorithm $\mathtt{Sampling\_Alg}$, which performs sampling on the space of $\{0,1\}^d$ based on the predicted weight $\widetilde{\wb}$ in the output embedding of the transformer.

\begin{algorithm}[H]
\caption{Sampling algorithm for in-context linear regression with binary coefficient}\label{alg:_sampling_alg_binary}
\begin{algorithmic}[1]
  \STATE \textbf{Input:} token embedding $\widetilde{\hb}$, coefficient sparsity $k\in[d]$.
  \STATE Initialize $\wb  \leftarrow  \mathbf{0}_d$ 
  \STATE Extract the coefficient $\widetilde{\wb}$ from $\widetilde{\hb}$, i.e., $\widetilde{\wb} = (\widetilde{\hb})_{d+2:2d+1}$ (see Proposition~\ref{prop:_construction})
  \STATE Compute predicted distribution $p = \mathtt{ClipNorm}(\widetilde{\wb})$ (see \eqref{eq:_sample_prob})
  \STATE Sample $k$ different indices $(e_1,\dots,e_k)\subset [d]$ based on $p$ without replacement (see \eqref{eq:_sample_discrete})\label{line:_sample}
  \STATE Assign corresponding indices of $\wb$ to 1:  $w_{e_\ell} = 1$ for each $e_\ell\in\{e_1,\cdots,e_k\}$
  \STATE \textbf{Output:} $\hb:=(\boldsymbol{0}, 0, \wb, 1)^\top$.
\end{algorithmic}
\end{algorithm}

In the above sampling procedure, the function $\mathtt{ClipNorm}(\cdot)$ first clips each element in $\widetilde{\wb}$ to be non-negative and then normalizes the resulting vector such that its elements sum to 1, i.e.,  
\begin{align}
    \big(\mathtt{ClipNorm}(\widetilde{\wb})\big)_i:= \frac{\max\{\widetilde{w}_i,0\}}{\sum_{i'=1}^d\max\{\widetilde{w}_{i'},0\}}.\label{eq:_sample_prob}
\end{align}
This mimics the generation of the probability distribution over the vocabulary set using softmax operation.
Then algorithm~\ref{alg:_sampling_alg_binary} mimics the decoding process of real-world LLMs by sampling discrete tokens according to such a distribution. 
More specifically, given the distribution $p$, we sample the (embedded) next token $\wb$ as a $k$-sparse vector with non-zero coordinates sampled from $p$ according to 
\begin{align}
    e_1\sim p, \,\,e_2\sim p(\cdot|e_2\neq e_1),\,\,\cdots, \,\, e_k\sim p(\cdot|e_k\notin \{e_1,\cdots,e_{k-1}\}).\label{eq:_sample_discrete}
\end{align}
We treat the vector sparsity $k$ as a fixed parameter satisfying $1 \leq k < d$, with $k$ typically set to $1$ in practice. 
Such a discrete nature of these coefficients enables us to consider the method of majority vote among the sampling-based test-time computing strategies in Definition~\ref{def:_test_time_computing}. 
In this work, we compare majority vote to a baseline inference mechanism based on greedy decoding which does not utilize random sampling.


\paragraph{Baseline: greedy decoding.}  
The baseline test-time computing method we consider is the greedy decoding algorithm. 
In the decoding step, instead of sampling $k$ items based on $p$ as depicted in Algorithm~\ref{alg:_sampling_alg_binary} (Line~\ref{line:_sample}), we opt to choose $k$ items with the highest $k$ probabilities under $p$ and set the corresponding indices of $\wb$ to 1. 
This mirrors the greedy decoding algorithm commonly used in practice.
We notice that such an algorithm does not introduce randomness into the decoding procedure and is not a sampling-based test-time computing technique in Definition~\ref{def:_test_time_computing}.
We denote the resulting prediction after $t$ reasoning steps as $\wb_{\mathtt{greedy}}$.

\paragraph{Majority vote.} Thanks to the discrete nature of the coefficients, we are able to apply the $\mathtt{Occur}(\cdot)$ function to candidate answers and select the one with the highest frequency in order to perform majority vote (see Definition~\ref{def:_test_time_computing}).
We denote the resulting prediction after sampling $N$ reasoning paths of length $t$ as $\wb_{\mathtt{mv}}$.


\paragraph{}

\textcolor{purple}{[Present numerical experiment results of (i) greedy decoding (ii) majority vote.]}


==> ArXiv/tex/binary.tex <==
\section{Analysis for In-context Binary Sparse Linear Regression}\label{sec:binary_analysis}

In this section, we establish the theoretical analysis of the test-time computing techniques for the binary sparse in-context linear regression task (Section~\ref{subsec:_binary}).
We first clarify several notations used throughout this section.
We denote the coefficient reasoned by greedy decoding mechanism by $\wb_t^{\mathtt{greedy}}$, and the prediction reasoned by majority vote with reasoning length $t$ and sampling number $N$ as $\wb_{t, N}^{\mathtt{mv}}$. 
% For the binary task, we fix $\eta = 1/n$, which is optimal for single-step gradient descent. 
% Thus, $\hat{\wb}_t = \tilde{\wb}_{t-1} - \frac{1}{n}(\Xb \Xb^\top \wb_{t-1} - \Xb \Yb^\top)$. 
% We sample the next weight $\tilde{\wb}_t$ based on $p_{\hat{\wb}_t}$ , 
% Due to the Markov property of the intermediate predictions $\{\wb_t,\wb_{t-1},\dots,\wb_0\}$ (due to Proposition~\ref{prop:_construction}), 
% We define the simplified notation $p(\wb\mid\wb') := \PP(\wb_t = \wb \mid \wb_{t-1} = \wb', \cD)$ and 
We define the simplified notation $p(\wb_t = \wb) := \PP(\wb_t = \wb \mid \wb_{0}, \cD)$ to denote the probability of obtaining weight $\wb$ after $t$ reasoning steps using Algorithm~\ref{alg:_sampling_alg_binary} conditioning on the initial state $\wb_{0}$ and the in-context dataset in a single reasoning path.
Our strategy of studying and comparing the test-time computing methods is to analyze the probability of perfectly recovering the true coefficient, i.e., $\mathbb{P}(\wb_t^{\mathtt{greedy}} = \wb^{\ast})$ and $\mathbb{P}(\wb_{t, N}^{\mathtt{mv}} = \wb^{\ast})$, where the probability is taken over the randomness of the in-context example and for the majority vote case it also includes the randomness of different reasoning paths.




% We first consider the case where $\PP(\wb_t = \wb^*) > \max\limits_{\wb' \in \cW\setminus\{\wb^{\ast}\}} \PP(\wb_t = \wb')$ state the sample complexity as follows:


Our first result shows that if in a single reasoning path the prediction $\wb_t$ has a probability of recovering the truth higher than that of recovering any other coefficient, then majority vote recovers the truth with a probability converging to $1$ exponentially fast.

\begin{proposition}[Sample complexity for majority vote] 
\label{th:sc_maj_vote}
    Consider the binary sparse linear regression task (Section~\ref{subsec:_binary}) and using majority vote with reasoning length $T$ and sampling number $N$. The final result $\wb_{t, N}^{\mathtt{mv}}$ can asymptotically recover the truth $\wb^*$ with probability $1$ given sufficient sample size $N$ if and only if for a single reasoning path it holds that
    \begin{align}
        \Delta_t:=p(\wb_t = \wb^*) - \max_{\wb' \in \cW\setminus\{\wb^{\ast}\}} p(\wb_t = \wb')>0,\label{eq:_recovery_condition}
    \end{align}
    and  under condition \eqref{eq:_recovery_condition}, it holds that
\begin{align} 
\PP\left(\wb_{t, N}^{\mathtt{mv}} = \wb^*\mid \wb_0, \cD\right) \geq  1 - |\cW|\cdot \exp\left(-\frac{N}{2}\cdot\Delta_t^2\right).
\end{align}
\end{proposition}

\begin{proof}[Proof of Proposition~\ref{th:sc_maj_vote}]
    Please refer to Appendix~\ref{subsec:_proof_thm_sc_maj_vote} for the proof of Proposition~\ref{th:sc_maj_vote}
\end{proof}

We remark that similar results of Proposition~\ref{th:sc_maj_vote} have also been proposed in \cite{wuInferenceScalingLaws2024}.
Here, we further provide a more detailed analysis for the majority vote algorithm in our binary sparse linear regression task, including the in-context example number $n$, reasoning length $t$, and compare it with the greedy search algorithm to emphasize the importance of the sample-then-select method.

Our main result is the following two theorems.
The first result is regarding the regime where we have sufficiently many in-context data $n$.

% {\bf [REWRITE THE THEOREM]}
% \begin{theorem}[Perfect recovery probability with sufficient in-context examples]
% \label{th:sc_sufficient_n}
%     Suppose that $n \geq (6k + 3\sigma)^4$, then the overall recovery probability of greedy decoding and majority vote are lower bounded as following:
%     \begin{itemize}
%         \item Greedy decoding: for any reasoning length $t\geq 1$, it holds that 
%         \begin{align}
%             \mathbb{P}\big(\wb^{\mathtt{greedy}}_t = \wb^{\ast}\big) \geq 1 -2d(d+2)\cdot \exp(-c n^{1/2}).
%         \end{align}
%         \item Majority vote: for any reasoning length $t\geq 1$ and sampling number $N\geq 1$, it holds that 
%         \begin{align}
%             \mathbb{P}\left(\wb_{t, N}^{\mathtt{mv}} = \wb^{\ast}\right) \geq \left(1-2d(d+2)\cdot \exp(-c n^{1/2})\right)\cdot \left(1 - \square  \right), \quad \textcolor{purple}{\text{plug in $p_1^{\ast}$ and $p_2^{\ast}$}}
%         \end{align}
%     \end{itemize}
%     % with probability at least $1 -2d(d+2)\exp(-c n^{1/2})$ over the randomness of the in-context dataset for some absolute constant $c>0$, both the prediction of greedy decoding and the majority will perfectly recover the true coefficient for any reasoning length $t\geq 1$ (given sufficient number of sample path for majority vote).
% % \begin{equation}
% % \begin{aligned}
% % \wb_{t, N}^{\mathtt{mv}}  = \wb_t^{\mathtt{greedy}} = \wb^* , 
% % \end{aligned}
% % \end{equation}
% % and the sampling number $N$ is sufficient large, 
% \textcolor{gray}{Moreover, 
% \begin{equation}
% \begin{aligned}
% \Delta P_T \geq \frac{p^*_1}{p^*_1 + 1 - p^*_2} (1-  (p^*_2 - p^*_1)^{t-1} ).
% \end{aligned}
% \end{equation}
% Where 
% \begin{equation}\begin{aligned}
% p^*_1 &= (1 - \frac{2k + \sigma}{n^{1/4} -(2k + \sigma)}) \frac{1}{|\cW|}, \\
% p^*_2 &= (1 - \frac{\sigma}{n^{1/4} - \sigma}) (\frac{n^{1/4} - \sigma}{n^{1/4} - \sigma + d \sigma})^{k}.
% \end{aligned}\end{equation}}
% \end{theorem}

\begin{theorem}[Perfect recovery probability with sufficient in-context examples]
\label{th:sc_sufficient_n}
    Suppose that $n \geq (6k + 3\sigma)^4$, then the overall recovery probability of greedy decoding and majority vote are lower bounded as following:
    \begin{itemize}
        \item Greedy decoding: for any reasoning length $t\geq 1$, it holds that 
        \begin{align}
            \mathbb{P}\big(\wb^{\mathtt{greedy}}_t = \wb^{\ast}\big) \geq 1 -2d(d+2)\cdot \exp(-c n^{1/2}).
        \end{align}
        \item Majority vote: for any reasoning length $t\geq 1$ and sampling number $N\geq 1$, it holds that 
        \begin{align}
            \mathbb{P}\left(\wb_{t, N}^{\mathtt{mv}} = \wb^{\ast}\right) \geq \left(1-2d(d+2)\cdot \exp(-c n^{1/2})\right)\cdot \left(1 - |\cW| \cdot \exp{(-2\Delta_t^2 N/2)}  \right), \quad \textcolor{purple}{\text{plug in $p_1^{\ast}$ and $p_2^{\ast}$}}
        \end{align}
    \end{itemize}
    Where $1> \Delta_t > 0$ for all $t \geq 1$, moreover, 
    \begin{equation}\begin{aligned}
    \Delta_t &\geq \frac{p_{\mathtt{trans}}}{p_{\mathtt{trans}} + 1 - p_{\mathtt{recurr}}} (1-  (p_{\mathtt{recurr}} - p_{\mathtt{trans}})^{t-1} ).\\
    p_{\mathtt{trans}} &= (1 - \frac{2k + \sigma}{n^{1/4} -(2k + \sigma)}) \frac{1}{d^k}, \\
    p_{\mathtt{recurr}} &= (1 - \frac{\sigma}{n^{1/4} - \sigma}) (\frac{n^{1/4} - \sigma}{n^{1/4} - \sigma + d \sigma})^{k}.
    \end{aligned}\end{equation}
\end{theorem}

\autoref{th:sc_sufficient_n}  establishes lower bounds on the recovery accuracy for both greedy search and majority vote. The accuracy improves exponentially with the number of in-context examples. For majority vote, since $1 > \Delta_t > 0$ for all $t \geq 1$, as with sufficient sample size ($N \rightarrow \infty$), we have $\mathbb{P}\left(\wb_{t, \infty}^{\mathtt{mv}} = \wb^{\ast}\right) \geq \left(1-2d(d+2)\cdot \exp(-c n^{1/2})\right)$. This bound matches that of greedy decoding $ \mathbb{P}\big(\wb^{\mathtt{greedy}}_t = \wb^{\ast}\big) $, and both algorithms achieve perfect accuracy given sufficient in-context examples $n$. Moreover, $p_{\mathtt{recurr}} > p_{\mathtt{trans}}$ since $\frac{n^{1/4} - \sigma}{n^{1/4} - \sigma + d \sigma} > \frac1d$ holds for $d > 1, \frac{\sigma}{n^{1/4}} < 1/3$. In particular, when $\sigma = 0$, we have $p_{\mathtt{recurr}} = 1$ and $p_{\mathtt{trans}} > \frac{2}{3d^k}$, ensuring that $\Delta_t$ converges to 1 as $t \rightarrow \infty$.

While real-world language models and our experimental results demonstrate that majority vote is more robust with a limited sample size, we next provide a analysis of limited in-context examples. We consider the case where $n = 1$ and $k = 1$, with only one in-context example $(\xb, \wb^\top \xb + \epsilon)$. Although this may be an oversimplification, we believe such a case can provide valuable insights into the robustness of the majority vote.

\begin{theorem}[Majority Vote Outperforms Greedy Search in the Case of Limited In-context Examples] \label{th:sc_limited_n} 
    Consider the case where $n = k = 1, \sigma = 0$, and denote the in-context example as $(\xb, \wb^\top \xb )$.
    
For majority vote algorithm, there exists a $\zeta > 0$ such that for reasoning steps $T > \frac{2\ln{1/2}}{\ln{1 - \zeta}}$ and  sufficient large sampling number $N$ it holds that 
\begin{equation} \begin{aligned} 
\wb_{t, N}^{\mathtt{mv}} = \wb^*,
\end{aligned} \end{equation} 
with probability at least $1 - \frac{1}{2^{d-1}}$.

For greedy search algorithm, it hold that
\begin{equation} \begin{aligned} 
\wb_t^{\mathtt{greedy}} \neq \wb^*,
\end{aligned} \end{equation} 
with probability at least $1 - \frac{1}{2^{d-1}} - \frac2d$.
\end{theorem}

\autoref{th:sc_limited_n} shows that with limited in-context examples, the majority vote can perform well while the greedy search would fail. We emphasize that the noise should be small enough; otherwise, $\wb^*$ may not be the optimal solution due to the limited in-context examples, making it impossible to recover the original $\wb^*$ due to the limited in-context example, so here we consider the case $\sigma = 0$.

Finally, we provide the overall accuracy with increasing reasoning length:

\begin{theorem}[Majority Vote Convergence Rate with Reasoning Length $T$] 
\label{th:cr_d_2} 
    Consider the case where $k = 1, d = 2$, denote the in-context example as $\Xb,\Yb$ with reasoning step $T$. Suppose $\PP(\wb\mid\wb')> 0 \, \forall \wb,\wb' \in \cW$  then 
\begin{equation} \begin{aligned} 
    \PP(\wb_t = \wb) = \PP(\wb_{\infty} = \wb) - \cO(\mu^{-T}), 
\end{aligned} \end{equation}

where $\PP(\wb_{\infty} = \wb^*)$ denotes the stationary distribution corresponding to the Markov transition matrix $\{\PP(\wb\mid\wb')\}_{\wb,\wb' \in \cW}$, and $\mu$ is a constant dependent on in-context example $(\Xb,\Yb)$. 
\end{theorem}

\autoref{th:cr_d_2} consider the case $k = 1, d = 2$ as we assume real world language model tend to choose from few potential answers. Note that different $\wb \in \cW$ shares the same trend $\cO(\mu^{-T})$, this insight can help us understand the inference process of LLMs.

==> ArXiv/tex/continuous.tex <==
\section{Analysis of In-context Linear Regression with Continuous Coefficient}\label{sec:continuous_analysis}



In this section, we establish the theoretical analysis of the test-time computing techniques for the in-context linear regression task with continuous coefficients (Section~\ref{subsec:_continuous}).
We consider the following setups for theoretical analysis. 
Recall that the in-context examples $(\xb_i,y_i)$ are independently sampled from the joint distribution $\cD_{\wb^{\ast}}$. 
We measure the performance of the regression coefficient $\wb$ reasoned using the transformer through test-time computation via its population risk in the population data distribution $\cD$, i.e., 
\begin{align}
    L_{\cD_{\wb^{\ast}}}(\wb):= \frac{1}{2}\cdot\mathbb{E}_{(\xb,y)\sim \cD_{\wb^{\ast}}}\left[\big(y - \xb^\top\wb\big)^2\right].
\end{align}
Equivalently, we can consider the following excess risk, 
\begin{align}
    \cE(\wb):=L_{\cD_{\wb^{\ast}}}(\wb) - \inf_{\wb'\in\RR^d} L_{\cD_{\wb^{\ast}}}(\wb) = \frac{1}{2}\cdot \|\wb - \wb^{\ast}\|_{\Hb}^2,\quad \Hb:= \mathbb{E}_{\xb\sim \cD}\left[\xb\xb^\top\right].
\end{align}
To facilitate the presentation, we introduce the following notations. 
We denote the sample covariance matrix of the in-context data as $\boldsymbol{\Sigma} := n^{-1}\Xb^\top\Xb\in\RR^{d\times d}$, and we denote the gram matrix of the in-context data as $\Ab := \Xb\Xb^\top\in\RR^{n\times n}$. 
We denote the collection of label noise in the in-context data as $\boldsymbol{\epsilon} := \yb - \Xb\wb^{\ast}$. 
We also denote the eigenvalues of the population covariance matrix $\Hb$ as $\{\lambda_i\}_{1\leq i\leq d}$, where we sort these eigenvalues in a non-increasing order.

Our analysis relies on the following standard assumptions on the data distribution \citep{bartlett2020benign}.

% \textcolor{purple}{[Here I stick to the convention that $\Xb\in\RR^{n\times d}$. 
% Let's adapt the notation to this convention for the transformer part.]}


\begin{assumption}[Data distribution]\label{ass:_data_distribution}
    We assume the following on the in-context data distribution $\cD_{\wb^{\ast}}$: 
    \begin{enumerate}[left=0mm]
        \item The columns of $\Hb^{-1/2}\xb$ are independent and $1$-subGaussian; 
        \item The labels are generated according to $y = \xb^\top\wb^{\ast} + \epsilon$, where the label noise $\epsilon$ is independent of $\xb$ and  satisfies $\mathbb{E}[\epsilon] = 0$ and $\mathbb{E}[\epsilon^2] = \sigma_{\epsilon}^2$ for some constant $\sigma_{\epsilon}>0$;
        \item The true coefficient $\wb^{\ast}$ follows the Gaussian prior, i.e., $\wb^{\ast}\sim \cN(\boldsymbol{0},\omega^2\cdot\Ib_d)$ for some constant $\omega>0$.
    \end{enumerate}
\end{assumption}

In the following, we first establish the excess risk bound for the baseline algorithm, i.e., in-context inference via vanilla multi-step GD \eqref{eq:_w_gd}.
After that, we present the analysis for sampling-based test-time computing methods and showcase the regime where keeping increasing the test time compute would result in better excess risk bounds compared to the baseline deterministic method, demonstrating the power of scaling up test-time computation in a principled manner in the task of in-context linear regression.


\paragraph{Baseline: multi-step GD with CoT.}

A baseline of test-time computing performed by the transformer for the linear regression task is vanilla multi-step gradient descent, i.e., \eqref{eq:_w_gd}. 
The following result gives the excess risk bound for such a test-time computing algorithm.

\begin{theorem}[Excess risk of vanilla multi-step GD with CoT]\label{thm:_gd_continuous}
    Under Assumption~\ref{ass:_data_distribution}, taking the step size $\eta\leq \|\Hb\|_2^{-1}$ and CoT length $t$, with probability at least $1-1/\mathrm{poly}(n)$, it holds that 
    \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast}}\left[\mathcal{E}(\wb_{\mathtt{GD}})\right]\lesssim \omega^2\cdot\Bigg(\frac{\widetilde{\lambda}^2}{n^2}\cdot \sum_{1\leq i\leq k^{\ast}} \frac{1}{\lambda_i} + \sum_{k^{\ast}<i\leq d}\lambda_i\Bigg) + \sigma^2_{\epsilon}\cdot\Bigg(\frac{k^{\ast}}{n} + \frac{n}{\widetilde{\lambda}^2}\cdot\sum_{k^{\ast}<i\leq d}\lambda_i^2\Bigg),
    \end{align}
    where the quantities $k^{\ast}$ and $\widetilde{\lambda}$ are defined as following respectively,
    \begin{align}
        k^{\ast} := \min\Bigg\{1\leq k\leq d: n\lambda_{k+1}\leq\frac{n}{\eta t} + \sum_{k<i\leq d} \lambda_i\Bigg\},\quad \widetilde{\lambda}:=\frac{n}{\eta t} + \sum_{k^{\ast} < i\leq d}\lambda_i.\label{eq:_k_lambda_vanilla}
    \end{align}
\end{theorem}


\begin{proof}[Proof of Theorem~\ref{thm:_gd_continuous}]
    Please refer to Appendix~\ref{subsec:_proof_thm_gd_continuous} for a proof of Theorem~\ref{thm:_gd_continuous}.
\end{proof}




\begin{corollary}\label{cor:_gd_continuous_polynomial_decay}
    Under the same assumptions and setups as in Theorem~\ref{thm:_gd_continuous}, by additionally assuming that the spectrum of $\Hb$ satisfies polynomially decaying, i.e., $\lambda_i = i^{-(r+1)}$ for some constant $r\geq 1$, then for any reasoning path length $t\lesssim \eta(r+1)^{(r+1)/2}d^{(r+1)/2}$, with probability at least $1-1/\mathrm{poly}(n)$, it holds that 
    \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast}}\left[\mathcal{E}(\wb_{\mathtt{GD}})\right]\lesssim \omega^2\cdot\left(\frac{1}{t\eta}\right)^{\frac{r}{r+1}} + \frac{\sigma_{\epsilon}^2}{n}\cdot (t\eta)^{\frac{1}{r+1}}.
    \end{align}
\end{corollary}



\begin{proof}[Proof of Corollary~\ref{cor:_gd_continuous_polynomial_decay}]
    Please refer to Appendix~\ref{subsec:proof_cor_gd_continuous_polynomial_decay} for a proof of Corollary~\ref{cor:_gd_continuous_polynomial_decay}.
\end{proof}



\paragraph{Aggregating by averaging.} 
In this situation, the final regression coefficient reasoned by the transformer test-time computing under the budget of CoT length $t$ and reasoning path number $N$ is explicitly given by
\begin{align}
    \wb_{\texttt{avg}}:=\frac{1}{N}\sum_{j=1}^N \wb^{(j)}_t,\quad \label{eq:_continuous_aggregating_w}
\end{align}
where each random reasoning path $\{\wb_{\ell}^{(j)}\}_{1\leq\ell \leq t}$ is independently and identically generated according to Definition~\ref{def:_inference_mechanism} via a transformer satisfying Proposition~\ref{prop:_construction} and the sampling method Algorithm~\ref{alg:_sampling_alg_continuous}.
We give separate results for the two choices of the noise transformation function $\phi_{\bxi}(\cdot)$ in Examples~\ref{exp:_constant} and \ref{exp:_linear}.


\begin{theorem}[Excess risk of noisy multi-step GD with CoT and averaging]\label{thm:_average_continuous}Under Assumption~\ref{ass:_data_distribution}, taking the step size $\eta\leq \|\Hb\|_2^{-1}$ and CoT length $t$, we have the following risk bounds for \eqref{eq:_continuous_aggregating_w}.
\begin{enumerate}[left=0mm]
\item Constant noise transformation function (Example~\ref{exp:_constant}): with probability at least $1-1/\mathrm{poly}(n)$, 
    \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast}}\left[\mathcal{E}(\wb_{\mathtt{GD}})\right]\lesssim \omega^2\cdot\Bigg(\frac{\widetilde{\lambda}^2}{n^2}\cdot \sum_{1\leq i\leq k^{\ast}} \frac{1}{\lambda_i} + \sum_{k^{\ast}<i\leq d}\lambda_i\Bigg) + \sigma^2_{\epsilon}\cdot\Bigg(\frac{k^{\ast}}{n} + \frac{n}{\widetilde{\lambda}^2}\cdot\sum_{k^{\ast}<i\leq d}\lambda_i^2\Bigg),
    \end{align}
    where the quantities $k^{\ast}$ and $\widetilde{\lambda}$ are defined as the same as \eqref{eq:_k_lambda_vanilla};
\item Linear noise transformation function (Example~\ref{exp:_linear}): taking the noise variance $\sigma^2\asymp d^{-1}$ and the reasoning path length $t>\sigma^{-2}\cdot \log 2$, with probability at least $1-1/\mathrm{poly}(n)$, 
    \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast},\bxi}\left[\mathcal{E}(\wb_{\mathtt{avg}})\right]\lesssim \omega^2\!\cdot\!\Bigg(\frac{(\widetilde{\lambda}^{\mathrm{Bias}})^2}{n^2}\cdot \!\!\!\!\sum_{1\leq i\leq k^{\ast}_{\mathrm{Bias}}} \!\frac{1}{\lambda_i} + \!\!\!\!\sum_{k^{\ast}_{\mathrm{Bias}}<i\leq d}\!\lambda_i\Bigg) + \sigma^2_{\epsilon}\!\cdot\!\Bigg(\frac{k^{\ast}_{\mathrm{Var}}}{n} + \frac{n}{(\widetilde{\lambda}^{\mathrm{Var}})^2}\cdot\!\!\!\!\sum_{k^{\ast}_{\mathrm{Var}}<i\leq d}\!\lambda_i^2\Bigg) + \delta_{N,t},
    \end{align}
    where the quantities $\widetilde{\lambda}^{\mathrm{Bias}}$, $\widetilde{\lambda}^{\mathrm{Var}}$, $k^{\ast}_{\mathrm{Bias}}$, and $k^{\ast}_{\mathrm{Var}}$ are defined as following respectively,
    \begin{align}
        k^{\ast}_{(\diamondsuit)} := \min\Bigg\{k\in[d]: n\lambda_{k+1}\leq\widetilde{\lambda}_{\mathrm{effect}}^{(\diamondsuit)} + \!\!\sum_{k<i\leq d} \lambda_i\Bigg\},\quad \widetilde{\lambda}^{(\diamondsuit)}:=\widetilde{\lambda}_{\mathrm{effect}}^{(\diamondsuit)}   +\!\!\! \sum_{k^{\ast} < i\leq d}\lambda_i, \quad \mathrm{for}\,\,(\diamondsuit)\in\{\mathrm{Bias}, \mathrm{Var}\},
    \end{align}
    with $\widetilde{\lambda}_{\mathrm{effect}}^{\mathrm{Bias}} $ and $\widetilde{\lambda}_{\mathrm{effect}}^{\mathrm{Var}} $ defined as,
    \begin{align}
        \widetilde{\lambda}_{\mathrm{effect}}^{\mathrm{Bias}}  := \frac{n}{\eta}\cdot \left(\frac{2}{t} + \frac{\sigma^2}{1-\sigma^2}\left(1+\frac{2}{t}\right)\right),\quad \widetilde{\lambda}_{\mathrm{effect}}^{\mathrm{Var}}  := \frac{\sigma^2n}{(1-\sigma^2)\eta},
    \end{align}
    and the quantity $\delta_{N,t}$, a fluctuation term caused by random sampling of $N$ times, is given by 
    \begin{align}
        \delta_{N,t}:=.
    \end{align}
    \end{enumerate}
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:_average_continuous}]
    Please refer to Appendix~\ref{subsec:_proof_thm_average_continuous} for a proof of Theorem~\ref{thm:_average_continuous}.
\end{proof}


\begin{corollary}\label{cor:_average_continuous}
     Under the same assumptions and setups as in Theorem~\ref{thm:_average_continuous},  additionally assuming that the spectrum of $\Hb$ satisfies polynomially decaying, i.e., $\lambda_i = i^{-(r+1)}$ for some constant $r\geq 0$.
     \begin{enumerate}[left=0mm]
         \item Constant noise transformation function (Example~\ref{exp:_constant}): taking the  reasoning path length $t\lesssim \eta (r+1)^{(r+2)/2}n^{(r+1)/2}$ and the sampling path number $N\geq \textcolor{red}{(TODO)}$ with probability at least $1-1/\mathrm{poly}(n)$, 
             \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast}, \bxi}\left[\mathcal{E}(\wb_{\mathtt{avg}})\right]\lesssim \omega^2\cdot\left(\frac{1}{t\eta}\right)^{\frac{r}{r+1}} + \frac{\sigma_{\epsilon}^2}{n}\cdot (t\eta)^{\frac{1}{r+1}}.
    \end{align}
         \item Linear noise transformation function (Example~\ref{exp:_linear}): taking the noise variance $\sigma^2\asymp d^{-1}$, the reasoning path length $\sigma^{-2}\cdot \log 2<t\lesssim \eta (r+1)^{(r+2)/2}n^{(r+1)/2}$, and the sampling path number $N\geq \textcolor{red}{(TODO)}$, with probability at least $1-1/\mathrm{poly}(n)$, 
             \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast},\bxi}\left[\mathcal{E}(\wb_{\mathtt{avg}})\right]\lesssim \omega^2\cdot\left(\frac{1}{\eta}\cdot \left(\frac{2}{t} + \frac{\sigma^2}{1-\sigma^2}\left(1+\frac{2}{t}\right)\right)\right)^{\frac{r}{r+1}} + \frac{\sigma_{\epsilon}^2}{n}\cdot\left(\frac{\eta\cdot(1-\sigma^2)}{\sigma^2}\right)^{\frac{1}{r+1}}.
    \end{align}
     \end{enumerate}
\end{corollary}



\begin{proof}[Proof of Corollary~\ref{cor:_average_continuous}]
    Please refer to Appendix~\ref{subsec:_proof_cor_average_continuous} for a proof of Corollary~\ref{cor:_average_continuous}.
\end{proof}


\begin{remark}
    Considering the same settings of Corollaries~\ref{cor:_gd_continuous_polynomial_decay} and \ref{cor:_average_continuous}, choosing the in-context data number $n$,  sampling noise$\sigma$, and reparametrizing the reasoning path length $t$ as 
    \begin{align}
        n\asymp \eta d,\quad \sigma^{2}\asymp d^{-1},\quad t = \widetilde{t}\cdot\sigma^{-2},\label{eq:_regime}
    \end{align}
    risk bounds for the vanilla multi-step GD with CoT method and the sample average method (using linear noise transformation function (Example~\ref{exp:_linear})) as following, 
    \begin{align}
        \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast}}\left[\mathcal{E}(\wb_{\mathtt{GD}})\right] \lesssim \widetilde{t}^{\frac{1}{r+1}} \cdot \sigma_{\epsilon}^2\cdot\left(\frac{1}{\eta d}\right)^{\frac{r}{r+1}},\quad \mathbb{E}_{\boldsymbol{\epsilon},\wb^{\ast},\bxi}\left[\mathcal{E}(\wb_{\mathtt{avg}})\right] \lesssim \big(\omega^2 + \sigma_{\epsilon}^2\big)\cdot\left(\frac{1}{\eta d}\right)^{\frac{r}{r+1}}.
    \end{align}
    Notice that by the conditions in Corollaries~\ref{cor:_gd_continuous_polynomial_decay} and \ref{cor:_average_continuous}, all the above conclusions hold when $t = \widetilde{t}\cdot\sigma^{-2}$ is not exceeding the order of $\eta(r+1)^{(r+1)/2}n^{(r+1)/2}$, which, under the parameter regime \eqref{eq:_regime}, translates to $\widetilde{t} \lesssim d^{(r-1)/2}$.
    Thus we are able to observe that in the high-dimensional regime, vanilla GD method has the disadvantage of harmful overfitting to the label noise when the effective reasoning path length $\widetilde{t}$ is increasing, while the sampling-based test-time computing method does not. 
\end{remark}




\paragraph{Aggregating by Best-of-N.}



==> ArXiv/tex/experiments.tex <==
\section{Experiments}
\subsection{Validation for Theoretical Analysis}

\begin{figure*}
\vskip -.1in
\centering
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=0.845\textwidth]{icml2025/figures/continuous_exp_new.pdf}
\end{subfigure}%[width=.8\linewidth]

\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=0.845\textwidth]{icml2025/figures/binary_exp.pdf}
\end{subfigure}%[width=.8\linewidth]
\caption{Numerical experiments on in-context linear regression with continuous coefficients  (\textit{above, a-d}) and binary coefficients (\textit{below, e-h}).}
\label{fig:add_exp}
\vskip -.1in
\end{figure*}

In the previous section, we provided detailed analyses for in-context linear regression with continuous/binary coefficients. Here, we validate our theoretical findings through numerical experiments. For the continuous case, we examine the effects of varying $\sigma_{data}$ and $\sigma_{coeff}$. Our results demonstrate that with average aggregation, constant noise provides no performance improvement, while linear noise reduces test loss given sufficient sample size, confirming \autoref{}. Furthermore, when decoding with a reward model, even constant noise yields consistent performance improvements as sample numbers increase, validating Theorem \autoref{}.

For the binary sparse coefficient case, we observe from \autoref{fig:add_exp} (e) that with sufficient examples, both greedy search and majority voting achieve perfect accuracy, supporting \autoref{th:sc_sufficient_n}. From \autoref{fig:add_exp} (f) we find that when setting $n=1$ and $d = 10, \sigma_{data} = 0$,  with sufficiently large reasoning length $T$, majority voting achieves high accuracy, while greedy search maintains approximately $2/d = 0.2$ accuracy, consistent with \autoref{th:sc_limited_n}. We fit the relationship between accuracy $\mathtt{Acc}$ and sample number $n$ using $\mathtt{Acc} = \alpha_{T} - \beta_{T} e^{-\nu_T N}$ for given $T$. The results, shown in \autoref{fig:add_exp} (g) and (h), not only validate \autoref{th:sc_maj_vote} but also suggest practical applications for real-world LLM inference.


\subsection{Insights for LLM Inference}

Our theoretical analysis reveals two critical terms $\mathcal{O}(e^{-(\Delta P_T)^2 N/2})$ and $\mathcal{O}(e^{-\mu T})$ for the overall accuracy $\mathtt{Acc}_T$ and probability gap $\Delta P_T$. These findings can provide valuable insights into real-world LLM inference.

To begin, we can observe that $\Delta P_T$ changes with the number of reasoning steps $T$ in $\mathcal{O}(e^{-\mu T})$. This can be described as:

\begin{equation} \begin{aligned} \label{eq:fit_p_n}
\Delta P_T &\approx \gamma - \kappa e^{-\mu T} 
\end{aligned} \end{equation}

Specifically, for sampling number of $N = 1$, based on \autoref{th:cr_d_2}, here we assume we can directly express the overall accuracy as:

 \begin{equation} \begin{aligned}\label{eq:fit_p_n_1}
\mathtt{Acc}(T,1) &\approx \gamma' - \kappa' e^{-\mu T}.
 \end{aligned} \end{equation}

Note that \autoref{eq:fit_p_n_1} and \autoref{eq:fit_p_n} shares the same $\mu$. To predict the final accuracy for a given sampling number $N$, here we introduce two additional parameters $(\alpha_{(T,N)}, \beta_{(T,N)})$ and formulate $\mathtt{Acc}(T,N)$ as:

\begin{equation} \begin{aligned} \label{eq:fit_acc_t_n}
\mathtt{Acc}(T,N) &\approx \alpha_{(T,N)} - \beta_{(T,N)} e^{-(\Delta P_T)^2 N/2}
\end{aligned} \end{equation}
 
Due to our limited sample number $N$, $\alpha_{(T,N)}$ and $\beta_{(T,N)}$ need to depend on both $N$ and $T$ to capture the nuanced relationship with $\mathtt{Acc}_T$. To effectively fit Eq~\ref{eq:fit_p_n}, \ref{eq:fit_p_n_1} and \ref{eq:fit_acc_t_n}, based on the fitting results onn \autoref{fig:add_exp} (g) and (h), we further make two assumptions:
\begin{itemize}
    \item When $T$ is fixed, then  Eq~\ref{eq:fit_acc_t_n} can be approximated by:
        \begin{equation} \begin{aligned}\label{eq:fit_acc_fix_t}
        \mathtt{Acc}(T,N) &\approx \alpha_{T} - \beta_{T} e^{-(\Delta P_T)^2 N/2}.
        \end{aligned} \end{equation}
    \item When $N$ is fixed, then Eq~\ref{eq:fit_acc_t_n} can be approximated by:
        \begin{equation} \begin{aligned}\label{eq:fit_acc_fix_n}
        \mathtt{Acc}(T,N) &\approx \alpha_{N} - \beta_{N} e^{-(\Delta P_T)^2 N/2}.
        \end{aligned} \end{equation}
\end{itemize}

This analysis enables us to predict model's high test-time computation performance using data from low-computation, resulting our Low-Cost-to-High Prediction algorithm \ref{alg:predicte_acc}, we validate our algorithm on GSM8K and a subset of MATH datasets,  details can be found in \autoref{appdix:exp_details}. The results in \autoref{fig:gsm8k_math_fit} demonstrate that our algorithm successfully predicts model performance at high computational costs using only data from settings with relatively low reasoning tokens $T$ or sampling numbers $N$.
 
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml2025/figures/fit_analysis.pdf}}
\caption{Utilizing data with low computational costs to forecast results for high computational costs. Where $\bigstar$ denotes predicted results and $\newmoon$ denotes the data utilized.}
\label{fig:gsm8k_math_fit}
\end{center}
\vskip -0.2in
\end{figure}

==> ArXiv/tex/introduction.tex <==
\section{Introduction}

Transformer-based \citep{vaswani2017attention} large language models (LLMs) have demonstrated impressive general-purpose capabilities, representing state-of-the-art architectures in natural language processing \citep{dubey2024llama,guo2025deepseek,achiam2023gpt} and increasingly in other domains such as computer vision \citep{peebles2023scalable,agarwal2025cosmos}.
% and also advancing theoretical analysis of their underlying mechanisms \cite{gargWhatCanTransformers2023, vonoswaldTransformersLearnIncontext2023}. 
While scaling laws for LLM training have described their performance with respect to the model size, data size, and training time, e.g., \cite{kaplan2020scaling}, leveraging and scaling up additional test-time computation of the pretrained LLMs has recently demonstrated great potential for further enhancing their reasoning capabilities \citep{o1, yue2024inference,wuInferenceScalingLaws2024,snellScalingLLMTestTime2024}. 
Recent research indicates that increasing test-time computation during language model inference, such as generating additional intermediate thoughts \citep{wei2022chain} or sampling multiple candidate answers and aggregating to obtain the best one \citep{cobbe2021training, wangSelfConsistencyImprovesChain2023}, can significantly improve the performance of the LLM.
However, despite the success of scaling up test-time computing for LLMs reasoning, the theoretical understanding of transformer models for such successes remain quite limited.
\textcolor{red}{also need to introduce what's test-time computation, mention reasoning, cot, mcts, also mention the concept of length of thoughts, samples, etc.}

% \begin{figure}[t!]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml2025/figures/overview.pdf}}
% \caption{Comparison between real-world LLM's inference (above) and our designed sampling framework (below). By injecting random noise with reward model, the loss decreases initially with increasing sample size, then increases, aligning well with the real-world LLM inference with a reward model shown above. Through sampling binary coefficients, the model exhibits a similar trend with LLM for majority vote. }
% \label{fig:gsm8k_sparse_comp}
% \end{center}
% \vskip -0.2in
% \end{figure}
% \begin{figure}[t!]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml2025/figures/overview_new.pdf}}
% \caption{Comparison between real-world LLM's inference (above) and our designed sampling framework (below). Our framework simulates language model decoding through noise injection and binary coefficient sampling, exhibiting trends similar to real-world LLMs' inference, Details can be found in \autoref{appdix:exp_details} }
% \label{fig:gsm8k_sparse_comp}
% \end{center}
% \vskip -0.2in
% \end{figure}

Due to the success of LLMs itself, a huge body of recent theory works has emerged, aiming at understanding the hidden mechanisms of transformer, seeking to explain the model's capabilities in memorization \citep{mahdaviMemorizationCapacityMultiHead2023,kimProvableMemorizationCapacity2023}, in-context learning (ICL) \citep{vonoswaldTransformersLearnIncontext2023,zhang2023trained}, function approximation power \citep{takakuraApproximationEstimationAbility2023,malachAutoRegressiveNextTokenPredictors2023}, algorithm simulation  \citep{chen2024can,fu2023transformers,liu2024learn}, and the training dynamics \citep{yangInContextLearningRepresentations2024,zhang2023trained,chen2024training} for  transformers initialized from scratch, to name a few.
\textcolor{red}{need to be more specific, clearly mention the works consider the linear transformer and linear setting, so that matching the last sentence in the first paragraph. also mention the iclr paper??}

However, these works typically focus transformer models with deterministic decoding procedures, where the model output is fixed for a given prompt. 
In practice, many  inference techniques for scaling up test-time computing, such as majority voting \citep{wangSelfConsistencyImprovesChain2023}, best-of-N sampling (BoN) \citep{cobbe2021training}, and tree of thoughts (ToT) \citep{yao2024tree}, rely on probabilistic sampling procedures in real-world LLMs: given a prompt, the model predicts subsequent tokens by first computing a distribution over potential candidates and then sampling from it. This gap between the theoretical setups and the real-world LLM behavior hinders us towards understanding and analyzing of the success of transformer test-time computation.



% In this work, we aim to bridge the gap between practical language model inference and theoretical transformer analysis, providing initial theoretical insights into transformer test-time computation. Specifically, we examine the in-context linear regression task with continuous/binary coefficients, where data is generated by a sparse coefficient $\wb^* \in \RR^d$(continues case) or $\wb^* \in \{0,1\}^d$ with $||\wb^*||_0 = k < d$, This task captures the sparsity properties observed in real-world language models\cite{li2022lazy} and has been widely adopted in theoretical analyses\cite{bai2024transformers,chen2024transformers,liu2024learn}. We simulate LLMs' sampling decoding procedure by injecting random noise (continuous case) or conducting discrete sampling (binary case) based on the model's original output, using the processed tokens for subsequent steps. We then conduct theoretical analysis towards test-time computation of transformers based on our reasoning framework. The main contributions of this paper are highlighted as follows:



\subsection{Our Contributions}
In this work, we aim to make the first step towards bridge such a gap between the language model inference with test-time computing scaling and theoretical transformer model analysis, providing initial theoretical insights into the empirical success.
Our contributions are three folds.

\paragraph{A framework of analyzing sampling-based test-time computing techniques for transformers.}

Specifically, we examine the in-context linear regression task with continuous/binary coefficients,
simulate LLMs' sampling decoding procedure by injecting random noise (continuous case) or conducting discrete sampling (binary case) based on the model's original output, using the processed tokens for subsequent sampling decoding steps. 

\paragraph{Theoretical analysis of test-time scaling law.}
% We take an initial step toward bridging the gap between practical language model inference and theoretical transformer analysis by incorporating randomness and sampling. Our framework simulates language model decoding through noise injection and binary coefficient sampling, exhibiting trends similar to real-world LLMs' inference, as demonstrated in \autoref{fig:gsm8k_sparse_comp}
Through our framework, we conduct detailed analysis of how test-time computation plays a role in our reasoning framework, including reasoning steps and sampling number, which can be applied to widely adopted inference techniques such as majority voting, best-of-N sampling, and chain-of-thought prompting.

\paragraph{Experimental demonstrations and insights for LLM inference.}
Our theoretical analysis provides insights for real-world LLM inference, suggesting the potential to utilize data from low computational cost scenarios to predict model performance under high computational costs.



\subsection{Related Works}


\paragraph{Scaling test-time computing in LLMs.}
Scaling test-time computing has demonstrated tremendous empirical success in LLMs, especially for reasoning tasks \citep{o1}.
Recent research on increasing test-time computing in LLMs primarily focuses on the following two aspects \citep{snell2024scaling}: (i) generating longer reasoning paths with more tokens, including chain-of-thought (CoT) prompting that elicits intermediate reasoning steps \citep{wei2022chain,kojima2022large} and self-refinement methods that iterate on previously generated content \citep{madaan2303self, saunders2022self,kumar2024training}; and (ii) generating multiple potential reasoning paths and selecting the optimal one through the methods such as consistency-based selection \citep{wangSelfConsistencyImprovesChain2023}, reward-guided choosing \citep{stiennon2020learning, liu2020learning, cobbe2021training,dong2023raft}, reasoning tree search \citep{yao2024tree,zhou2023language}, etc.
Empirical studies demonstrate that increased test-time computation consistently improves model performance \cite{snellScalingLLMTestTime2024,yue2024inference,o1}, suggesting the existence of inference scaling laws \citep{wuInferenceScalingLaws2024}.
Nevertheless, the theoretical analysis of inference-time computing and its scaling law remains quite open.

\paragraph{Theoretical understanding of transformer test-time computing.}
Inspired by the empirical success of the inference-time computing techniques of LLMs, recently there has been a few works trying to demystify the mechanism behind it and uncover the fundamental power of test-time computing through analysis on theoretical tasks and simple transformer models.
Both \cite{wen2024sparse, kim2024transformers} consider how to train a one-layer transformer that utilizes chain-of-thought reasoning to efficiently solve the $k$-parity learning task, which provably improve over the same one without using CoT reasoning. 
\cite{hu2024unveiling} studies the statistical properties of CoT prompting and its variants including majority vote and tree-of-thought (ToT). 
However, their analysis is model agnostic and does not consider concrete transformer models compared with our work. 
The mostly related to our paper is the work of \cite{anonymous2025transformers} who considers the training of a one-layer transformer to solve in-context linear regression task with continuous coefficient.
They show that the transformer can be well trained to perform vanilla multi-step GD with CoT. 
However, the fundamental difference between the study of \cite{anonymous2025transformers, wen2024sparse, kim2024transformers} and ours is that we propose to include randomness in the inference stage of the transformer models we study, which then allows us to go further and study more sophisticated test-time computing methods that requires sampling multiple reasoning or CoT paths and select the aggregated ones based on certain rules.

% \cite{wen2024sparse, kim2024transformers, hu2024unveiling, anonymous2025transformers}

\paragraph{Theoretical analysis of in-context learning by transformers.}
In-context learning (ICL) \citep{brown2020language} is a key capability of LLMs which means that the model is able to answer a new query provided with a few query-answer demonstrations of the similar tasks without updating the model parameters.
The empirical success of ICL methods has sparked a long line of theoretical research for the ICL ability of transformers. 
Most of these theoretical research builds on the in-context learning framework of  \cite{gargWhatCanTransformers2023}, where input-output pairs are formalized as $\{(\xb_i,f(\xb_i))\}_{i = 1}^{n}$, and the model (typically, transformers) is required to learn the unknown function $f(\cdot)$ from the context without updating the parameters. This framework enables theoretical analysis of transformers across multiple dimensions: expressive power \citep{bai2024transformers,guoHowTransformersLearn2023}, mechanistic understanding \citep{giannouHowWellCan2024, vonoswaldTransformersLearnIncontext2023, ahn2023transformers}, and training dynamics \citep{zhang2023trained, huangContextConvergenceTransformers2023, chen2024training}. While most existing research treats transformer decoding as a deterministic process, theoretical understanding of test-time computation for transformer ICL remains in its infancy.

==> ArXiv/tex/preliminaries.tex <==
\subsection{Preliminaries and More Backgrounds}

In this section, we introduce the problem setups.
Firstly, we formally introduce the background of transformers and its inference mechanism, especially the \emph{sampling-based} techniques to scale up test-time computation for performance improvement. 
Secondly, we introduce the theoretical task -- in-context linear regression -- that we aim to solve for the study of test-time computing. 

\subsubsection{Transformer and Sampling-based Test-time Computing}\label{subsec:_transformer_test_time_compute}

A transformer \citep{vaswani2017attention} can be understood as an auto-regressive sequence-to-sequence model that maps a token sequence of any length to a distribution of the next token, i.e., $p(x_{t+1}|x_t,\cdots,x_1)$. 
The typical mechanism for choosing the probability of the next token $x_{t+1}$ is to map the hidden embedding of the last token $x_t$ after the transformer hidden layers to a softmax distribution over the vocabulary space $\cV$. 

The above inference mechanism can be abstracted in the following way. 
Given the current input sequence embedding $\Hb_t = (\hb_1,\cdots,\hb_t)\in\mathbb{R}^{d_{\mathrm{e}}\times t}$, one \emph{iteratively} performs the following two steps: 
\begin{itemize}
    \item Compute and extract the hidden state for the last position $t$, i.e., $\widetilde{\hb}_t = \mathtt{TF}_{\theta}(\Hb_t)$, where $\mathtt{TF}_{\theta}$ denotes the stacked transformer blocks in the whole architecture.
    \item Sample the next token $x_{t+1}$ (and thus the embedding of the next token $\hb_{t+1}$) based on a probability distribution returned by a sampling algorithm inputted with $\widetilde{\hb}_t$, i.e., $\hb_{t+1} \leftarrow \mathtt{Sampling\_Alg}(\widetilde{\hb}_t)$.
\end{itemize}


\paragraph{Sampling-based test-time compute.}

As previously introduced, the probabilistic nature of the computation procedure can introduce randomness into the inference process, which is key to an array of techniques for scaling up test-time computing in order to boost the performance of large language models for various tasks, including Best-of-N sampling (BoN) \citep{stiennon2020learning, nakano2021webgpt, dong2023raft}, majority vote \citep{wang2022self}, etc.
Notably, the BoN method typically samples $N$ independent reasoning trajectories through the above decoding mechanism, and proposes to choose the one that achieves the highest value of a given reward model. 
The reward model could be given or trained independently.
Also, the majority vote, or the self-consistency method, typically first samples $N$ independent reasoning paths
and then chooses the answer that is the most consistent across the $N$ results, 
by marginalizing out the intermediate steps. 

\subsubsection{Theoretical Task: In-context Linear Regression.}\label{subsec:_theoretical_task}

To initiate the theoretical study of how sampling-based test-time computing scaling can boost the performance of transformers for task solving, we focus on a widely adopted problem setup of \emph{in-context linear regression} \citep{akyurek2022learning, von2023transformers, zhang2023trained} as a playground. 
In-context learning (ICL \cite{brown2020language}) refers to the inference-time capability of auto-regressive models to infer the answer of a query given a few demonstrations of the task. 
In-context linear regression instantiates such a task to linear regression problems. 
Specifically, we consider the following general setup: 
\begin{align}
    \wb^{\ast}\sim p_{\wb}(\cdot),\quad  (\xb_i, y_i)\sim \cD_{\wb^{\ast}},\quad   y_i = \xb_i^\top \wb^{\ast} + \epsilon_i,\quad  \forall 1\leq i\leq n,\label{eq:_in_context_linear_regression}
\end{align}
where $p_{\wb}$ denotes the prior distribution of the regression tasks, and $n\in\NN$ is the size of the in-context dataset.
% $d$ is the ambient dimension of the covariates, $\sigma^2_{\epsilon}>0$ is the variance of the label noise, 
The goal of in-context linear regression is to use transformers to make predictions regarding the true label $\xb_{\mathrm{query}}^\top \wb^{\ast}$ associated with another covariate $\xb_{\mathrm{query}}\sim \cN(0,\Ib_d)$ when prompted with the in-context dataset $(\xb_1,y_1,\cdots,\xb_n,y_n)$ concatenated with the query $\xb_{\mathrm{query}}$.
Towards such a goal, this work aims to establish a theoretical framework that allows one to principally investigate how sampling-based techniques for scaling up test-time computing could benefit the predictions, thus boosting the performance of solving the task.







==> icml2025/sections/abstract.tex <==
\begin{abstract}
Using more test-time computation during language model inference, such as generating more intermediate thoughts or sampling multiple candidate answers, has proven effective in significantly improving model performance. This paper takes an initial step toward bridging the gap between practical language model inference and theoretical transformer analysis by incorporating randomness and sampling. We focus on in-context linear regression with continuous/binary coefficients, where our framework simulates language model decoding through noise injection and binary coefficient sampling. Through this framework, we provide detailed analyses of widely adopted inference techniques. Supported by empirical results, our theoretical framework and analysis demonstrate the potential for offering new insights into understanding inference behaviors in real-world language models.
% Our theoretical analyses, supported by empirical results, offer new insights into understanding inference behaviors in real-world language models.
\end{abstract}

==> icml2025/sections/binary.tex <==

% \subsection{Analysis for Binary Sparse Linear Regression}


Here we denote the majority vote result with reasoning length $t$ and sampling number $N$ as $\wb_t^{\mathtt{maj}\cdot N}$, and the result of greedy search with reasoning length $t$ as $\wb_t^{\mathtt{greedy}}$. For the binary task, we fix $\eta = 1/n$, which is optimal for single-step gradient descent. Thus, $\hat{\wb}_t = \tilde{\wb}_{t-1} - \frac{1}{n}(\Xb \Xb^\top \wb_{t-1} - \Xb \Yb^\top)$. We sample the next weight $\tilde{\wb}_t$ based on $p_{\hat{\wb}_t}$ , due to the Markov property of $\{\wb_t,\wb_{t-1},\dots,\wb_0\}$, we use the notation $\PP(\wb\mid\wb') = \PP(\wb_t = \wb \mid \wb_{t-1} = \wb')$ and $\PP(\wb_t = \wb) = \PP(\wb_t = \wb \mid \wb_{0})$ to denote the probability of sampling  weight $\wb$ conditioned on the last state $\wb_{t-1}= \wb'$ and the initial state $\wb_{0} = \mathbf{0}$. We first consider the case where $\PP(\wb_t = \wb^*) > \max\limits_{\wb' \in \cW_{/\wb^*}} \PP(\wb_t = \wb')$ state the sample complexity as follows:

\begin{theorem}[Sample Complexity for Majority Vote] 
\label{th:sc_maj_vote}
    Consider a binary sparse linear regression task using majority vote with reasoning length $T$. The final result $\wb_t^{\mathtt{maj}\cdot N}$ converges to $\wb^*$ with sufficient sample size $N$ iif $\PP(\wb_T = \wb^*) > \max\limits_{\wb' \in \cW_{/\wb^*}} \PP(\wb_T = \wb')$, and  
\begin{equation} \begin{aligned} 
\PP(\wb_t^{\mathtt{maj}\cdot N} = \wb^*) = 1 - \cO(e^{-(\Delta P_T)^2 N/2}), 
\end{aligned} \end{equation} 
where $\Delta P_T = \PP(\wb_T = \wb^*) - \max\limits_{\wb' \in \cW_{/\wb^*}} \PP(\wb_T = \wb')$.
\end{theorem}

\autoref{th:sc_maj_vote} states that the majority vote converges to the highest probability weight exponentially with the sample size $N$. Similar results have been stated in \cite{wuInferenceScalingLaws2024}; here, we provide a more detailed analysis for the majority vote algorithm based on our binary sparse linear regression task, including the in-context example number $n$, reasoning length $T$, and comparison with the greedy search algorithm to emphasize the importance of sample-then-select algorithms, resulting in the following theorems:

\begin{theorem}[Perfect Accuracy for Greedy Search and Majority Vote with Sufficient In-context Examples]
\label{th:sc_sufficient_n}
    Suppose $\frac{2k + \sigma}{n^{1/4}} < \frac12$ and sampling number $N$ is sufficient large, then it holds that
\begin{equation}
\begin{aligned}
\wb_t^{\mathtt{maj}\cdot N}  = \wb_t^{\mathtt{greedy}} = \wb^* , 
\end{aligned}
\end{equation}
with probability at least $1 -\delta $, where $\delta = 2(d^2 + d) e^{-c n^{1/2}} $ and $c$ is a constant number, moreover, 
\begin{equation}
\begin{aligned}
\Delta P_T \geq \frac{p^*_1}{p^*_1 + 1 - p^*_2} (1-  (p^*_2 - p^*_1)^{t-1} ).
\end{aligned}
\end{equation}
Where 
\begin{equation}\begin{aligned}
p^*_1 &= (1 - \frac{2k + \sigma}{n^{1/4} -(2k + \sigma)}) \frac{1}{|\cW|}, \\
p^*_2 &= (1 - \frac{\sigma}{n^{1/4} - \sigma}) (\frac{n^{1/4} - \sigma}{n^{1/4} - \sigma + d \sigma})^{k}.
\end{aligned}\end{equation}
\end{theorem}

\autoref{th:sc_sufficient_n} provides the lower bound of accuracy for both greedy search and majority vote. The accuracy increases exponentially with the number of in-context examples. Specifically, with sufficient in-context examples, $\delta$ will approach zero, and both algorithms will achieve perfect accuracy.

While real-world language models and our experimental results demonstrate that majority vote is more robust with a limited sample size, we next provide a analysis of limited in-context examples. We consider the case where $n = 1$ and $k = 1$, with only one in-context example $(\xb, \wb^\top \xb + \epsilon)$. Although this may be an oversimplification, we believe such a case can provide valuable insights into the robustness of the majority vote.

\begin{theorem}[Majority Vote Outperforms Greedy Search in the Case of Limited In-context Examples] \label{th:sc_limited_n} 
    Consider the case where $n = k = 1, \sigma = 0$, and denote the in-context example as $(\xb, \wb^\top \xb )$.
    
For majority vote algorithm, there exists a $\zeta > 0$ such that for reasoning steps $T > \frac{2\ln{1/2}}{\ln{1 - \zeta}}$ and  sufficient large sampling number $N$ it holds that 
\begin{equation} \begin{aligned} 
\wb_T^{\mathtt{maj}\cdot N} = \wb^*,
\end{aligned} \end{equation} 
with probability at least $1 - \frac{1}{2^{d-1}}$.

For greedy search algorithm, it hold that
\begin{equation} \begin{aligned} 
\wb_t^{\mathtt{greedy}} \neq \wb^*,
\end{aligned} \end{equation} 
with probability at least $1 - \frac{1}{2^{d-1}} - \frac2d$.
\end{theorem}

\autoref{th:sc_limited_n} shows that with limited in-context examples, the majority vote can perform well while the greedy search would fail. We emphasize that the noise should be small enough; otherwise, $\wb^*$ may not be the optimal solution due to the limited in-context examples, making it impossible to recover the original $\wb^*$ due to the limited in-context example, so here we consider the case $\sigma = 0$.

Finally, we provide the overall accuracy with increasing reasoning length:

\begin{theorem}[Majority Vote Convergence Rate with Reasoning Length $T$] 
\label{th:cr_d_2} 
    Consider the case where $k = 1, d = 2$, denote the in-context example as $\Xb,\Yb$ with reasoning step $T$. Suppose $\PP(\wb\mid\wb')> 0 \, \forall \wb,\wb' \in \cW$  then 
\begin{equation} \begin{aligned} 
    \PP(\wb_t = \wb) = \PP(\wb_{\infty} = \wb) - \cO(\mu^{-T}), 
\end{aligned} \end{equation}

where $\PP(\wb_{\infty} = \wb^*)$ denotes the stationary distribution corresponding to the Markov transition matrix $\{\PP(\wb\mid\wb')\}_{\wb,\wb' \in \cW}$, and $\mu$ is a constant dependent on in-context example $(\Xb,\Yb)$. 
\end{theorem}

\autoref{th:cr_d_2} consider the case $k = 1, d = 2$ as we assume real world language model tend to choose from few potential answers. Note that different $\wb \in \cW$ shares the same trend $\cO(\mu^{-T})$, this insight can help us understand the inference process of LLMs.

==> icml2025/sections/related_work.tex <==
% [OLD]

\textbf{Related Works.} Our work is related to recent works on \emph{scaling test-time computing in LLMs}, \emph{theory for transformer test-time computing}, and \emph{theory for transformer in-context learning}.
Due to space limit, we defer them to Appendix~\ref{sec:_related_work_continued}.

% [NEW]
% \textbf{Related Works.} Our work is connected to recent studies likw \emph{scaling test-time computing in LLMs} and \emph{theory for transformer ICL}. Further details are provided in Appendix~\ref{sec:_related_work_continued} due to space constraints.
% \vspace{-3.5mm}
% may move to appendix


% \section{Related Works}

% \textbf{Scaling Test-Time Computation for LLMs}
% Research on increasing test-time computation primarily focuses on two aspects: (1) generating longer reasoning paths with more tokens, including chain-of-thought prompting that elicits intermediate reasoning steps \cite{wei2022chain,kojima2022large} and self-refinement methods that iterate on previously generated content \cite{madaan2303self, saunders2022self}; (2) exploring multiple potential reasoning paths and selecting the optimal one, through methods such as consistency-based selection \cite{wangSelfConsistencyImprovesChain2023}, reward-guided choosing \cite{liu2020learning, cobbe2021training}, and reasoning tree search \cite{yao2024tree,zhou2023language}. Empirical studies demonstrate that increased test-time computation consistently improves model performance \cite{snellScalingLLMTestTime2024,yue2024inference}, suggesting the existence of inference scaling laws \cite{wuInferenceScalingLaws2024} for LLMs.

% \textbf{In-context Learning}
% The empirical success of in-context learning has sparked theoretical analyses of transformer architectures. Most research builds on the in-context learning framework \cite{gargWhatCanTransformers2023}, where input-output pairs are formalized as ${(\xb_i,f(\xb_i))}_{i = 1}^{n}$, and models required to learn the unknown function $f(\cdot)$ from the context. This framework enables theoretical analysis of transformers across multiple dimensions: expressive power \cite{bai2024transformers,guoHowTransformersLearn2023}, mechanistic understanding \cite{giannouHowWellCan2024, vonoswaldTransformersLearnIncontext2023, ahn2023transformers}, and training dynamics \cite{huangContextConvergenceTransformers2023, zhang2023trained}. While most existing research treats transformer decoding as a deterministic process, theoretical understanding of test-time computation for transformers remains in its infancy.
